What You See is Not What You Get: The Role of Email Presentation in Phishing Susceptibility

Phishing is one of the most prevalent social engineering attacks that targets both organizations and individuals. It is crucial to understand how email presentation impacts users' reactions to phishing attacks. We speculated that the device and email presentation may play a role, and, in particular, that how links are shown might influence susceptibility. Collaborating with the IT Services unit of a large organization doing a phishing training exercise, we conducted a study to explore the effects of the device and the presentation of links. Our findings indicate that mobile device and computer users were equally likely to click on unmasked links, however mobile device users were more likely to click on masked links compared to computer users. These findings suggest that link presentation plays a significant role in users' susceptibility to phishing attacks.

==> Phishing Campaign study/cases.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Fri Feb 17 17:51:20 2023
\begin{table}[ht]
\centering
\begin{tabular}{|l|p{2cm}|r|r|c|r|}
  \hline
\bf Case & \bf Hypothesis & $\chi^2$ & \bf p value & $\phi$ & \bf resi \\ 
  \hline
Mov & H1: all & 5.0 & .025 & .06 & 1.39 \\ 
  Del & H1: all & 6.5 & .011 & .08 & 1.32 \\ 
   \hline
Mov & H1: raw only & $<$.01 & 0.927 & $<$.01 & -0.06 \\ 
  Del & H1: raw only & .6 & .424 & .04 & 0.39 \\ 
   \hline
Mov & H1: button only & 5.4 & .02 & .12 & 1.29 \\ 
  Del & H1: button only & 5.4 & .02 & .12 & 1.29 \\ 
   \hline
Mov & H1: hypertext only & 6.0 & .014 & .10 & 1.61 \\ 
  Del & H1: hypertext only & 3.1 & .08 & .09 & .86 \\ 
   \hline
Mov & H2: masked vs. raw & 34.8 & $<$.001 & .12 & 3.05 \\ 
  Del & H2: masked vs. raw & 32.8 & $<$.001 & .12 & 2.98 \\ 
   \hline
Mov & H2: button vs. raw & 17.4 & $<$.001 & .10 & 2.81 \\ 
  Del & H2: button vs. raw & 20.6 & $<$.001 & .12 & 2.97 \\ 
   \hline
Mov & H2: hypertext vs. raw & 41.3 & $<$.001 & .15 & 3.99 \\ 
  Del & H2: hypertext vs. raw & 36.6 & $<$.001 & .15 & 3.89 \\ 
   \hline
Mov & H3: button vs. hypertext & 5.2 & .023 & .05 & 1.40 \\ 
  Del & H3: button vs. hypertext & 2.8 & .092 & .04 & 1.10 \\ 
   \hline
\end{tabular}
\end{table}


